Confidence Intervals for Stochastic Arithmetic

Quantifying errors and losses due to the use of Floating-Point (FP) calculations in industrial scientific computing codes is an important part of the Verification, Validation and Uncertainty Quantification (VVUQ) process. Stochastic Arithmetic is one way to model and estimate FP losses of accuracy, which scales well to large, industrial codes. It exists in different flavors, such as CESTAC or MCA, implemented in various tools such as CADNA, Verificarlo or Verrou. These methodologies and tools are based on the idea that FP losses of accuracy can be modeled via randomness. Therefore, they share the same need to perform a statistical analysis of programs results in order to estimate the significance of the results. In this paper, we propose a framework to perform a solid statistical analysis of Stochastic Arithmetic. This framework unifies all existing definitions of the number of significant digits (CESTAC and MCA), and also proposes a new quantity of interest: the number of digits contributing to the accuracy of the results. Sound confidence intervals are provided for all estimators, both in the case of normally distributed results, and in the general case. The use of this framework is demonstrated by two case studies of large, industrial codes: Europlexus and code_aster.

==> schema.tex <==
\makeatletter%
  %
  % /header %
    %
    % /header/colors %
        \definecolor{colorA}{HTML}{377EB8}%
        \definecolor{colorB}{HTML}{E41A1C}%
        \definecolor{colorC}{HTML}{4DAF4A}%
        \definecolor{colorD}{HTML}{984EA3}%
        \definecolor{colorE}{HTML}{FF7F00}%
        \definecolor{colorF}{HTML}{A65628}%
        \definecolor{colorG}{HTML}{F781BF}%
        \definecolor{colorH}{HTML}{FFFF33}%
    %
    % /header/markers %
        \def\markerA{$+$}%
        \def\markerB{$\circ$}%
        \def\markerC{$\Box$}%
        \def\markerD{$\triangle$}%
        \def\markerE{$\times$}%
        \def\markerF{$\bullet$}%
        \def\markerG{$\blacksquare$}%
        \def\markerH{$\blacktriangle$}%
    %
    % /header/patterns %
        \tikzstyle{patternA}=[solid]%
        \tikzstyle{patternB}=[solid]%
        \tikzstyle{patternC}=[solid]%
        \tikzstyle{patternD}=[solid]%
        \tikzstyle{patternE}=[solid]%
        \tikzstyle{patternF}=[solid]%
        \tikzstyle{patternG}=[solid]%
        \tikzstyle{patternH}=[solid]%
    %
    % /header/thickness %
        \tikzstyle{thickA}=[thin]%
        \tikzstyle{thickB}=[very thick]%
        \tikzstyle{thickC}=[very thick]%
        \tikzstyle{thickD}=[very thick]%
        \tikzstyle{thickE}=[very thick]%
        \tikzstyle{thickF}=[very thick]%
        \tikzstyle{thickG}=[very thick]%
        \tikzstyle{thickH}=[very thick]%
  %
  % /background %
  \def\plotz@background{%
    %
    % /background/bbox %
      \fill[white](0.000000,0.000000)rectangle(160.000000,9.900000);%
    %
    % /background/grid %
    %
    % /background/legend %
  }%
  %
  % /lines %
  \def\plotz@lines{%
    \draw[fill=colorA](70.604948141803362,0.000000000000000)rectangle(76.322870604386438,4.000000000000000);%
    \draw[fill=colorA](76.322870604386438,0.000000000000000)rectangle(82.040793066969499,5.000000000000000);%
    \draw[fill=colorA](82.040793066969499,0.000000000000000)rectangle(87.758715529552575,4.000000000000000);%
    \draw[fill=colorA](87.758715529552575,0.000000000000000)rectangle(93.476637992135636,9.000000000000000);%
    \draw[fill=colorA](93.476637992135636,0.000000000000000)rectangle(99.194560454718712,7.000000000000000);%
    \draw[fill=colorA](99.194560454718712,0.000000000000000)rectangle(104.912482917301787,8.000000000000000);%
    \draw[fill=colorA](104.912482917301787,0.000000000000000)rectangle(110.630405379884849,5.000000000000000);%
    \draw[fill=colorA](110.630405379884849,0.000000000000000)rectangle(116.348327842467924,4.000000000000000);%
    \draw[fill=colorA](116.348327842467924,0.000000000000000)rectangle(122.066250305051000,1.000000000000000);%
    \draw[fill=colorA](122.066250305051000,0.000000000000000)rectangle(127.784172767634061,3.000000000000000);%
    \draw[colorB,patternA,thickA]%
      (0.000000000000000,0.000000001698395)%
    --(1.616161616161616,0.000000003463131)%
    --(3.232323232323232,0.000000006980035)%
    --(4.848484848484849,0.000000013906078)%
    --(6.464646464646465,0.000000027384832)%
    --(8.080808080808081,0.000000053305727)%
    --(9.696969696969697,0.000000102564253)%
    --(11.313131313131313,0.000000195063736)%
    --(12.929292929292929,0.000000366703810)%
    --(14.545454545454545,0.000000681416539)%
    --(16.161616161616163,0.000001251607868)%
    --(17.777777777777779,0.000002272386832)%
    --(19.393939393939394,0.000004078069366)%
    --(21.010101010101010,0.000007234113505)%
    --(22.626262626262626,0.000012684530414)%
    --(24.242424242424242,0.000021984765365)%
    --(25.858585858585858,0.000037664104064)%
    --(27.474747474747474,0.000063781071745)%
    --(29.090909090909090,0.000106761421958)%
    --(30.707070707070706,0.000176642520008)%
    --(32.323232323232325,0.000288891337405)%
    --(33.939393939393938,0.000467016422241)%
    --(35.555555555555557,0.000746256541036)%
    --(37.171717171717169,0.001178697912895)%
    --(38.787878787878789,0.001840243293270)%
    --(40.404040404040401,0.002839921516194)%
    --(42.020202020202021,0.004332073315045)%
    --(43.636363636363633,0.006531961602463)%
    --(45.252525252525253,0.009735310637097)%
    --(46.868686868686865,0.014342153608110)%
    --(48.484848484848484,0.020885135193631)%
    --(50.101010101010097,0.030062048944018)%
    --(51.717171717171716,0.042771869152424)%
    --(53.333333333333336,0.060152855293085)%
    --(54.949494949494948,0.083620474903788)%
    --(56.565656565656568,0.114901944353711)%
    --(58.181818181818180,0.156063194118466)%
    --(59.797979797979799,0.209523128502246)%
    --(61.414141414141412,0.278049305315812)%
    --(63.030303030303031,0.364728771594279)%
    --(64.646464646464651,0.472907932510991)%
    --(66.262626262626256,0.606096169364480)%
    --(67.878787878787875,0.767829590497160)%
    --(69.494949494949495,0.961493861539373)%
    --(71.111111111111114,1.190108487124349)%
    --(72.727272727272720,1.456079052663224)%
    --(74.343434343434339,1.760928495232932)%
    --(75.959595959595958,2.105023040411568)%
    --(77.575757575757578,2.487312495387402)%
    --(79.191919191919197,2.905107548710222)%
    --(80.808080808080803,3.353918024124507)%
    --(82.424242424242422,3.827375190695102)%
    --(84.040404040404042,4.317257938492669)%
    --(85.656565656565661,4.813636830950119)%
    --(87.272727272727266,5.305141982668043)%
    --(88.888888888888886,5.779350939640984)%
    --(90.505050505050505,6.223282097572613)%
    --(92.121212121212125,6.623968734599021)%
    --(93.737373737373730,6.969079606603367)%
    --(95.353535353535349,7.247545362824842)%
    --(96.969696969696969,7.450146701569939)%
    --(98.585858585858588,7.570020789294702)%
    --(100.202020202020194,7.603047174905812)%
    --(101.818181818181813,7.548082938068045)%
    --(103.434343434343432,7.407028356091293)%
    --(105.050505050505052,7.184717827581588)%
    --(106.666666666666671,6.888644784664478)%
    --(108.282828282828277,6.528542423934450)%
    --(109.898989898989896,6.115852965824447)%
    --(111.515151515151516,5.663125763877009)%
    --(113.131313131313135,5.183388277876225)%
    --(114.747474747474740,4.689533509729231)%
    --(116.363636363636360,4.193763254970584)%
    --(117.979797979797979,3.707119127123703)%
    --(119.595959595959599,3.239123743258471)%
    --(121.212121212121204,2.797543848069795)%
    --(122.828282828282823,2.388276637889633)%
    --(124.444444444444443,2.015351133083974)%
    --(126.060606060606062,1.681028911113975)%
    --(127.676767676767668,1.385983330320328)%
    --(129.292929292929301,1.129533709641913)%
    --(130.909090909090907,0.909910656640062)%
    --(132.525252525252512,0.724530498922195)%
    --(134.141414141414145,0.570260062537063)%
    --(135.757575757575751,0.443657276037598)%
    --(137.373737373737384,0.341177690302871)%
    --(138.989898989898990,0.259341492914105)%
    --(140.606060606060595,0.194859576207325)%
    --(142.222222222222229,0.144720437306910)%
    --(143.838383838383834,0.106242026019864)%
    --(145.454545454545439,0.077094107886692)%
    --(147.070707070707073,0.055297359756045)%
    --(148.686868686868678,0.039205407278057)%
    --(150.303030303030312,0.027475519273679)%
    --(151.919191919191917,0.019032867044198)%
    --(153.535353535353522,0.013032294451660)%
    --(155.151515151515156,0.008820555141190)%
    --(156.767676767676761,0.005901050347833)%
    --(158.383838383838395,0.003902303884283)%
    --(160.000000000000000,0.002550769513579)%
    ;%
  }%
  %
  % /foreground %
  \def\plotz@foreground{%
    %
    % /foreground/axes %
      \draw(0.000000000000000,0)--(160.000000000000000,0);%
      \draw(80.000000000000000,0)++(0,-2.000000em)node[anchor=north]{$x$};%
        \draw(0.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{0};%
        \draw(20.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{20};%
        \draw(40.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{40};%
        \draw(60.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{60};%
        \draw(80.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{80};%
        \draw(100.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{100};%
        \draw(120.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{120};%
        \draw(140.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{140};%
        \draw(160.000000000000000,0)++(0,0.5em)--++(0,-1em)%
           node[rotate=0.000000,anchor=north]{160};%
      \draw(0.000000000000000,0)--(0.000000000000000,9.900000000000000);%
      \draw(0.000000000000000,4.950000000000000)++(-2.400000em,0)node[anchor=east,rotate=90,anchor=south,inner sep=1em]{\# occurrences};%
        \draw(0.000000000000000,0.000000000000000)++(0.5em,0)--++(-1em,0)%
           node[rotate=0.000000,anchor=east]{0};%
        \draw(0.000000000000000,2.000000000000000)++(0.5em,0)--++(-1em,0)%
           node[rotate=0.000000,anchor=east]{2};%
        \draw(0.000000000000000,4.000000000000000)++(0.5em,0)--++(-1em,0)%
           node[rotate=0.000000,anchor=east]{4};%
        \draw(0.000000000000000,6.000000000000000)++(0.5em,0)--++(-1em,0)%
           node[rotate=0.000000,anchor=east]{6};%
        \draw(0.000000000000000,8.000000000000000)++(0.5em,0)--++(-1em,0)%
           node[rotate=0.000000,anchor=east]{8};%
    %
    % /foreground/legend %
        \draw[thick, dashed](1.000000e+02,0)--(1.000000e+02,9.900000e+00)%
        ++(2em,-1em)node[anchor=west](tmp){$\mu$};%
        \draw[->](tmp.west)--++(-2em,0);%
        \draw[thick, dashed](9.661789e+01,0)--(9.661789e+01,9.900000e+00)%
        ++(-2em,-1em)node[anchor=east](tmp){$\hat\mu$};%
        \draw[->](tmp.east)--++(2em,0);%
        \draw[thick,dashed](85,0)--(85,7.425000e+00)%
        ++(-2em,-1em)node[anchor=east](tmp){$x_{\text{ieee}}$};%
        \draw[->](tmp.east)--++(2em,0);%
  }%
  %
  % /legend %
  \def\plotz@legend{%
  }%
  %
  % /legendmargin %
  \def\plotz@legendmargin{%
  }%
  %
  % /scale %
    \def\plotz@scalex{1.666625}%
    \def\plotz@scaley{20.202020}%
\makeatother%

